Towards trustable SHAP scores

SHAP scores represent the proposed use of the well-known Shapley values in eXplainable Artificial Intelligence (XAI). Recent work has shown that the exact computation of SHAP scores can produce unsatisfactory results. Concretely, for some ML models, SHAP scores will mislead with respect to relative feature influence. To address these limitations, recently proposed alternatives exploit different axiomatic aggregations, all of which are defined in terms of abductive explanations. However, the proposed axiomatic aggregations are not Shapley values. This paper investigates how SHAP scores can be modified so as to extend axiomatic aggregations to the case of Shapley values in XAI. More importantly, the proposed new definition of SHAP scores avoids all the known cases where unsatisfactory results have been identified. The paper also characterizes the complexity of computing the novel definition of SHAP scores, highlighting families of classifiers for which computing these scores is tractable. Furthermore, the paper proposes modifications to the existing implementations of SHAP scores. These modifications eliminate some of the known limitations of SHAP scores, and have negligible impact in terms of performance.

==> figs/calcs.tex <==
\begin{figure*}[t]
  \begin{minipage}{0.35\linewidth}
    \begin{subfigure}[b]{1.0\linewidth} %\textwidth
      \centering
      \scalebox{0.875}{
        \renewcommand{\arraystretch}{1.15}
        \renewcommand{\tabcolsep}{0.575em}
        \input{./tabs/aexs}
      }
      \caption{Adversarial examples}\label{ex:calcs:aex}
    \end{subfigure}

    \begin{tabular}{c} ~~\\[-1.0pt] \end{tabular}
    
    \begin{subfigure}[b]{1.0\linewidth} %\textwidth
      %\begin{tabular}{c} ~~\\[0.0pt] \end{tabular}
      \centering
      \scalebox{0.875}{
        \renewcommand{\arraystretch}{1.15}
        \renewcommand{\tabcolsep}{0.575em}
        \input{./tabs/axps}
      }
      \caption{Abductive explanations}\label{ex:calcs:axp}
    \end{subfigure}
  \end{minipage}
  %
  \begin{minipage}{0.65\linewidth}
    \begin{subfigure}[b]{1.0\linewidth} %\textwidth
      \centering
      \scalebox{0.875}{
        \renewcommand{\arraystretch}{1.15}
        \renewcommand{\tabcolsep}{0.5em}
        \input{./tabs/svs}
      }
      %
      %\begin{tabular}{c} ~~\\[0.0pt] \end{tabular}
      %
      \caption{SHAP scores}\label{ex:calcs:svs}
    \end{subfigure}
  \end{minipage}
  %
  \caption{AExs, AXPs \& SHAP scores for the regression tree
    from~\cref{ex:tr:rt} and target sample $((1,1),1)$.
    For simplicity, parameterizations are elided.}
  \label{ex:calcs}
\end{figure*}


==> figs/runex.tex <==
\begin{figure*}[t]
  \begin{subfigure}[b]{0.4325\linewidth} %\textwidth

    \begin{tabular}{c} ~~\\[5pt] \end{tabular}

    \centering
    \scalebox{0.875}{
      \renewcommand{\arraystretch}{1.15}
      \renewcommand{\tabcolsep}{0.575em}
      \input{./tabs/tr01}
    }
    %
    %\begin{tabular}{c} ~~\\[-2pt] \end{tabular}
    %
    \caption{Tabular representation (TR)}
  \end{subfigure}
  %
  \begin{subfigure}[b]{0.2585\linewidth} %\textwidth
    \centering
    \scalebox{0.85}{
      \input{./texfigs/dt00}
    }
    \caption{Regression tree (RT)}
  \end{subfigure}
  %
  %
  \begin{subfigure}[b]{0.2775\linewidth} %\textwidth

    \begin{tabular}{c} ~~\\[5pt] \end{tabular}

    \centering
    \scalebox{0.875}{
      \renewcommand{\arraystretch}{1.15}
      \renewcommand{\tabcolsep}{0.575em}
      \input{./tabs/avg}
    }

    \begin{tabular}{c} ~~\\[-1.0pt] \end{tabular}

    \caption{Expected values} \label{ex:tr:rt:avg}
  \end{subfigure}
  %
  \caption{Simple regression tree model, 
    adapted from~\cite[Fig.~8.1]{james-bk17}. 
    The target sample is $((1,1),1)$.}
  \label{ex:tr:rt}
\end{figure*}


==> tabs/avg.tex <==
\renewcommand{\tabcolsep}{0.45em}
\begin{tabular}{ccc} \toprule
  $\fml{S}$ & $\msf{rows}(\fml{S})$ & $\cfn{e}(\fml{S})$
  \\ \toprule
  $\emptyset$ & $1,2,3,4$ & $1-\alpha$ \\
  $\{1\}$ & $3,4$ & $1$ \\
  $\{2\}$ & $2,4$ & $1+\alpha$ \\
  $\{1,2\}$ & $4$ & $1$
  \\ \bottomrule
\end{tabular}


==> tabs/svs.tex <==
\begin{tabular}{cccccc} \toprule
  \multicolumn{6}{c}{$i=1$} \\
  \toprule
  $\fml{S}$ & $\cf_e(\fml{S})$ & $\cf_e(\fml{S}\cup\{1\})$ &
  $\Delta_1(\fml{S})$ & $\varsigma(\fml{S})$ &
  $\varsigma(\fml{S})\times\Delta_1(\fml{S})$ \\
  \toprule
  $\emptyset$ & $1-\alpha$ & 1 & $\alpha$ & $\nfrac{1}{2}$ &
  $\nfrac{\alpha}{2}$ \\
  $\{2\}$ & $1+\alpha$ & 1 & $-\alpha$ & $\nfrac{1}{2}$ &
  $-\nfrac{\alpha}{2}$ \\
  \midrule
  \multicolumn{5}{r}{$\svn{E}(1)~~=$} & \multicolumn{1}{c}{0} \\
  \toprule
  \multicolumn{6}{c}{$i=2$} \\
  \toprule
  $\fml{S}$ & $\cfn{e}(\fml{S})$ & $\cfn{e}(\fml{S}\cup\{2\})$ &
  $\Delta_2(\fml{S})$ & $\varsigma(\fml{S})$ &
  $\varsigma(\fml{S})\times\Delta_2(\fml{S})$ \\
  \toprule
  $\emptyset$ & $1-\alpha$ & $1+\alpha$ & $2\alpha$ & $\nfrac{1}{2}$
  & $\alpha$ \\
  $\{1\}$ & 1 & 1 & 0 & $\nfrac{1}{2}$ & 0 \\
  \midrule
  \multicolumn{5}{r}{$\svn{E}(2)~~=$} & \multicolumn{1}{c}{$\alpha$} \\
  \bottomrule
\end{tabular}


==> tabs/tr01.tex <==
\renewcommand{\tabcolsep}{0.45em}
\begin{tabular}{cccccc} \toprule
  row & $x_1$ & $x_2$ & $\rho(\mbf{x})$ &
  \makecell{$\rho_a(\mbf{x})$\\$\alpha=\sfrac{1}{2}$} &
  \makecell{$\rho_b(\mbf{x})$\\$\alpha=\sfrac{1}{4}$}
  \\ \toprule
  1 & 0 & 0 & $1-6\alpha$ & $-2$ & $-\sfrac{1}{2}$ \\
  2 & 0 & 1 & $1+2\alpha$ & $2$ & $\sfrac{3}{2}$ \\
  3 & 1 & 0 & 1           & 1               & 1 \\
  \tikzmarknode{a}{4} & 1 & 1 & 1           & 1               & \tikzmarknode{b}{1}
  \\ \bottomrule
  \begin{tikzpicture}[overlay,remember picture]
    \node[draw=midblue, thin, xshift=-0.35pt, yshift=-0.35pt, inner
      sep=2.0pt, fit=(a) (b)] {};
  \end{tikzpicture}
\end{tabular}


==> texfigs/dt00.tex <==
% Concocted example
%%
%\tikzset{every label/.style={xshift=-0.35ex,
%  yshift=-5.25ex,
%  text width=1ex,
%  align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%
%\tikzset{tlabel/.style={xshift=0.25ex, yshift=1.75ex, text width=1ex,
%    align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%%\tikzset{every node/.style={---rectangle---}}
%
\forestset{
  BDT/.style={
    for tree={
      l=1.5cm,s sep=1.15cm,
      if n children=0{}{circle}, %rectangle
      %if n children=0{}{draw},
      draw=midblue,%draw=black,%
      text=midblue,%text=black,%
      edge={
        my edge
      },
      %if n=1{
      %  edge+={0 my edge},
      %}{},
      edge=thick,
      %font=\sffamily,
    }
  },
}
%
\begin{forest}
  BDT
  [{$x_1$}, label={[yshift=-6.875ex]{{\tiny1}}} 
    [{$x_2$}, label={[yshift=-6.875ex]{{\tiny2}}}, %xshift=-3.075ex,yshift=-3.5ex
      edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}}
      [\ncolor{\boldmath{$1-6\alpha$}}, label={[yshift=-5.25ex]{{\tiny4}}},
        edge label={node[midway,left,xshift=-0.5pt]
          {{\scriptsize$\in\{0\}$}}}, rectangle, fill={torange1!10} ]
      [\ncolor{\boldmath{$1+2\alpha$}}, label={[yshift=-5.25ex]{{\tiny5}}},
        edge label={node[midway,right,xshift=-0.575pt] {{\scriptsize$\in\{1\}$}}}, rectangle, fill={torange1!10} ]
    ]
    [\ncolor{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny3}}},
      edge={very thick,draw=tblue2}, edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
      rectangle, fill={torange1!10} ]
  ]
\end{forest}


==> texfigs/dt04.tex <==
% Concocted example
%%
%\tikzset{every label/.style={xshift=-0.35ex,
%  yshift=-5.25ex,
%  text width=1ex,
%  align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%
%\tikzset{tlabel/.style={xshift=0.25ex, yshift=1.75ex, text width=1ex,
%    align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%%\tikzset{every node/.style={---rectangle---}}
%
\forestset{
  BDT/.style={
    for tree={
      l=1.5cm,s sep=1.15cm,
      if n children=0{}{circle}, %rectangle
      %if n children=0{}{draw},
      draw=midblue,%draw=black,%
      text=midblue,%text=black,%
      edge={
        my edge
      },
      %if n=1{
      %  edge+={0 my edge},
      %}{},
      edge=thick,
      %font=\sffamily,
    }
  },
}
%
\begin{forest}
  BDT
  [{$x_1$}, label={[yshift=-6.875ex]{{\tiny1}}} 
    [{$x_4$}, label={[yshift=-6.875ex]{{\tiny2}}}, %xshift=-3.075ex,yshift=-3.5ex
      edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}}
      [\dghlight{\textbf{2}}, label={[yshift=-5.25ex]{{\tiny4}}},
        edge label={node[midway,left,xshift=-0.5pt]
          {{\scriptsize$\in\{0\}$}}}, rectangle, fill={tblue2!25} ]
      [\dghlight{\textbf{0}}, label={[yshift=-5.25ex]{{\tiny5}}},
            edge label={node[midway,right,xshift=-0.575pt] {{\scriptsize$\in\{1\}$}}}, rectangle, fill={tblue2!25} ]
    ]
    [{$x_2$}, label={[yshift=-6.875ex]{{\tiny3}}}, %xshift=-3.075ex,yshift=-3.5ex
      edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}}
      [{$x_3$}, label={[yshift=-6.875ex]{{\tiny6}}}, %xshift=-3.075ex,yshift=-3.5ex
        edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}}
        [\dghlight{\textbf{0}}, label={[yshift=-5.25ex]{{\tiny8}}},
          edge label={node[midway,left,xshift=-0.5pt]
            {{\scriptsize$\in\{0\}$}}}, rectangle, fill={tblue2!25} ]
        [\dghlight{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny9}}},
          edge label={node[midway,right,xshift=-0.575pt] {{\scriptsize$\in\{1\}$}}}, rectangle, fill={tblue2!25} ]
      ]
      [\dghlight{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny7}}},
        edge label={node[midway,right,xshift=-0.5pt] {{\scriptsize$\in\{1\}$}}},
        rectangle, fill={tblue2!20} ]
    ]
  ]
\end{forest}

